Depth Prompting for Sensor-Agnostic Depth Estimation

Dense depth maps have been used as a key element of visual perception tasks. There have been tremendous efforts to enhance the depth quality, ranging from optimization-based to learning-based methods. Despite the remarkable progress for a long time, their applicability in the real world is limited due to systematic measurement biases such as density, sensing pattern, and scan range. It is well-known that the biases make it difficult for these methods to achieve their generalization. We observe that learning a joint representation for input modalities (e.g., images and depth), which most recent methods adopt, is sensitive to the biases. In this work, we disentangle those modalities to mitigate the biases with prompt engineering. For this, we design a novel depth prompt module to allow the desirable feature representation according to new depth distributions from either sensor types or scene configurations. Our depth prompt can be embedded into foundation models for monocular depth estimation. Through this embedding process, our method helps the pretrained model to be free from restraint of depth scan range and to provide absolute scale depth maps. We demonstrate the effectiveness of our method through extensive evaluations. Source code is publicly available at https://github.com/JinhwiPark/DepthPrompting .

==> tables/rebuttal_SPR_comb.tex <==
% \begin{table}[t]
% % \LARGE
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c||ccc|ccc|ccc|ccc}
% \toprule
% % & Sparsity + Pattern& Pattern + Range & Sparsity + Range & ALL
%  & \multicolumn{3}{c}{Sparsity + Pattern} & \multicolumn{3}{c}{Pattern + Range} & \multicolumn{3}{c}{Sparsity + Range} & \multicolumn{3}{c}{ALL} \\ \midrule
%                   % & RMSE            & MAE             &\!\!DELTA1\!\!         & RMSE              & MAE               &\!\!DELTA1\!\!           & RMSE              & MAE               &\!\!DELTA1\!\!           & RMSE                & MAE                &\!\!DELTA1\!\!       \\ \midrule
% % CSPN              & 0.4902          & 0.3102          & 0.8323          & 0.1538            & 0.0802            & 0.9877            & 0.1108            & 0.0468            & 0.9937            & 0.7657              & 0.5401             & 0.6310                                  \\
% % S2D               & 1.3680          & 1.0730          & 0.3006          & 0.5608            & 0.3134            & 0.8827            & 0.4794            & 0.4331            & 0.6836            & 0.8988              & 0.6230             & 0.6265        \\
% % NLSPN             & 0.4639          & 0.3018          & 0.8554          & 0.1516            & 0.0758            & 0.9882            & 0.1136            & 0.0466            & 0.9933            & 1.2200              & 0.9202             & 0.3982   \\
% DySPN             & 0.4473          & 0.2700          & 0.8832          & 0.1487            & 0.0779            & \textbf{0.9887}   & 0.1088            & 0.0439            & 0.9935            & 0.6700              & 0.4117             & 0.7461   \\
% CostDCNet         & 0.4701          & 0.2946          & 0.8569          & 0.1458            & 0.0717            & 0.9883            & 0.1248            & 0.0557            & 0.9921            & 0.4164              & 0.2649             & 0.8955   \\
% % CompletionFormer  & 0.4776          & 0.2957          & 0.8510          & 0.1486            & 0.0754            & 0.9879            & 0.1183            & 0.0476            & 0.9925            & 0.8862              & 0.5993             & 0.6276   \\ \midrule
% % SpAgNet           & 0.7390          & 0.5784          & 0.6152          & 0.7692            & 0.6079            & 0.5783            & 0.6354            & 0.5335            & 0.5962            & 0.7293              & 0.5681             & 0.6205   \\ \midrule
% % Ours+Midas        & 0.4472          & 0.2787          & 0.8567          & 0.1722            & 0.0754            & 0.9827            & 0.1403            & 0.0549            & 0.9884            & 0.4478              & 0.2840             & 0.8608   \\
% Ours+KBR          & \textbf{0.3632} & \textbf{0.2282} & \textbf{0.8939} & 0.1503            & 0.0651            & 0.9865            & 0.1170            & 0.0449            & 0.9922            & 0.3133              & 0.1980             & 0.9434   \\
% Ours  & 0.3997          & 0.2418          & 0.8825          & \textbf{0.1453}   & \textbf{0.0634}   & 0.9874            & \textbf{0.1081}   & \textbf{0.0419}   & \textbf{0.9937}   & \textbf{0.2961}     & \textbf{0.1766}    & \textbf{0.9291}      \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-4mm}
% \caption{\JH{Case study on sensor biases (RMSE~/~MAE~/~DELTA1).}}
% \vspace{-4mm}
% \label{tab:SPR_comb}
% \end{table}



% \begin{table}[t]
% \Huge
% \centering
% \renewcommand{\arraystretch}{0.85}%
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c||c|c|c|c}
% \midrule
%           & ~~~{Sparsity+Pattern}~~~ & ~~~{Pattern+Range}~~~ & ~~~{Sparsity+Range~~~} & ~~~{ALL}~~~           \\ \cmidrule{2-5}
% CSPN      & 0.6235~/~0.3879           & 0.8917~/~0.6090          & 1.0060~/~0.7302          & 1.0010~/~0.7246          \\
% DYSPN     & 0.5665~/~0.3584           & 0.9580~/~0.6809          & 1.0270~/~0.7471          & 1.0290~/~0.7449          \\
% CostDCNet & 0.5573~/~0.3226           & 0.8878~/~0.5889          & 1.0060~/~0.5584          & 1.0100~/~0.7397          \\ 
% Ours      & \textbf{0.3181}~/~\textbf{0.2059}  & \textbf{0.5656}~/~\textbf{0.3584} & \textbf{0.6168}~/~\textbf{0.4511} & \textbf{0.6270}~/~\textbf{0.4500} \\ \midrule
% \end{tabular}%
% }
% \vspace{-8mm}
% \caption{Case study on multiple sensor biases (RMSE~/~MAE).}
% \vspace{-4mm}
%  \label{tab:SPR_comb}
% \end{table}

\begin{table}[t]
\Huge
\centering
\renewcommand{\arraystretch}{0.9}%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c||c|c|c|c@{}}
\midrule
          & ~~~{Sparsity+Pattern}~~~ & ~~~{Pattern+Range}~~~ & ~~~{Sparsity+Range~~~} & ~~~{ALL}~~~           \\ \cmidrule{2-5}
CSPN~[\textcolor{blue}{11}]      & 0.624~/~0.388           & 0.892~/~0.609          & 1.006~/~0.730          & 1.001~/~0.725          \\
DySPN~[\textcolor{blue}{37}]     & 0.567~/~0.358           & 0.958~/~0.681          & 1.027~/~0.747          & 1.029~/~0.745          \\
CostDCNet~[\textcolor{blue}{28}] & 0.557~/~0.323           & 0.888~/~0.589          & 1.006~/~0.558          & 1.010~/~0.740          \\ 
Ours      & \textbf{0.318}~/~\textbf{0.206}  & \textbf{0.566}~/~\textbf{0.358} & \textbf{0.617}~/~\textbf{0.451} & \textbf{0.627}~/~\textbf{0.450} \\ \midrule
\end{tabular}%
}
\vspace{-7.8mm}
\caption{Case study on multiple sensor biases (RMSE~/~MAE).}
\vspace{-4.3mm}
 \label{tab:SPR_comb}
\end{table}


==> tables/rebuttal_SpAgNet.tex <==
% \begin{table}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c||cccccccc||cccccccc}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NYU   (N)\\      KITTI (K)\end{tabular}} & \multicolumn{2}{c}{200 (N)} & \multicolumn{2}{c}{100 (N)} & \multicolumn{2}{c}{50 (N)} & \multicolumn{2}{c}{5 (N)} & \multicolumn{2}{c}{32 (K)}        & \multicolumn{2}{c}{16 (K)}        & \multicolumn{2}{c}{8 (K)}         & \multicolumn{2}{c}{4 (K)}         \\ \cmidrule{2-17}
%                                                                                     & RMSE              & REL     & RMSE            & REL       & RMSE         & REL         & RMSE        & REL         & RMSE            & MAE             & RMSE            & MAE             & RMSE            & MAE             & RMSE            & MAE             \\ \midrule
% SpAgNet                                                                             & 0.1550            & 0.0240  & 0.2090          & 0.0380    & 0.2720       & 0.0580      & 0.4670      & 0.1310      & 1.1642          & \textbf{0.3392}          & 1.8633          & 0.6069          & 2.6913          & 1.0872          & 3.5337          & 1.6226          \\
% Ours                                                                                & \textbf{0.1435}   &         & \textbf{0.1778} & \textbf{} & \textbf{}    & \textbf{}   & \textbf{}   & \textbf{}   & \textbf{1.1465} & 0.3472 & \textbf{1.3512} & \textbf{0.4134} & \textbf{1.6419} & \textbf{0.5470} & \textbf{1.9507} & \textbf{0.7629} \\ \bottomrule
% \end{tabular}%
% }
% \caption{Comparing results between ours and SpAgNet from [\textcolor{blue}{12}]}
% \label{tab:SpAgNet}
% \end{table}

\begin{table}[t]
% \LARGE
\centering
\renewcommand{\arraystretch}{0.9}%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c||@{}c@{}c@{}c@{}c@{}||@{}c@{}c@{}c@{}c@{}}
\toprule
               & 200 (N)           & 100 (N)         & 50 (N)      & 5 (N)     & ~32 (K)~                    & ~16 (K)~          & ~8 (K)~           &  ~4 (K)~         \\ \cmidrule{2-9}
SpAgNet        & 0.155            & 0.209          & 0.272      & 0.467     & 1.164                   & 1.863          & 2.691          & 3.534          \\
Ours           & ~\textbf{0.144$\pm$0.003}~   & ~\textbf{0.178$\pm$0.005}~ & ~\textbf{0.213$\pm$0.006}~   & ~\textbf{0.380$\pm$0.010}~  & ~\textbf{1.147}~          & ~\textbf{1.351}~ & ~\textbf{1.642}~ & ~\textbf{1.951}~ \\ \bottomrule
\end{tabular}
}
\vspace{-3.7mm}
    \caption{RMSE~(m) between ours and SpAgNet directly referred from the original paper~[\textcolor{blue}{12}] on NYU~(N) and KITTI~(K).}
\vspace{-4.1mm}
\label{tab:SpAgNet}
\end{table}

==> tables/rebuttal_fewshot_foundation.tex <==
% \begin{table}[t]
% % \Huge
% \centering
% \renewcommand{\arraystretch}{0.8}%
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c||cc|cc}
% \toprule
%       % & \multicolumn{2}{c}{NYU -\textgreater KITTI} & \multicolumn{2}{c}{KITTI -\textgreater NYU}\\ \midrule
%            & 64~(N$\rightarrow$ K)  & 8~(N$\rightarrow$ K)   & 500~(K$\rightarrow$ N) & 50  (K$\rightarrow$ N) \\ \midrule
% Ours+Midas & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000         \\
% Ours+KBR   & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000         \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-3.5mm}
% \caption{Few-shot evaluation w/o pretraining in depth completion.}
% \vspace{-4mm}
% \label{tab:few_foundation}
% \end{table}

% \begin{table}[t]
% % \Huge
% \centering
% \renewcommand{\arraystretch}{0.8}%
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c||c||cccc}
% \toprule
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}KITTI \\ $\downarrow$ \\ NYU\end{tabular}}& \# Lines   & 500             & 50              & 500             & 50              \\ \cmidrule{2-6}
%                         & Midas    & 0.1885 / 0.0839 & 0.8017 / 0.0517 & 0.2059 / 0.0971 & 0.1910 / 0.8623 \\
%                         & KBR      & 0.1769 / 0.0784 & 0.4153 / 0.2668 & 0.3103 / 0.2151 & 0.4971 / 0.3784 \\ \midrule
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}NYU \\ $\downarrow$ \\ KITTI\end{tabular}}& \# Samples & 64              & 8               & 64              & 8               \\ \cmidrule{2-6}
% & Midas    & 1.2780 / 0.3486 & 4.8571 / 2.5653 & 1.9273 / 0.5875 & 6.3762 / 3.6092 \\
%                         & KBR      & 1.2226 / 0.3324 & 4.2090 / 2.1382 & 1.8790 / 0.6192 & 5.1340 / 2.8451 \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-3.5mm}
% \caption{Few-shot cross-validation as in Tab.\textcolor{blue}{3}~(RMSE~/~MAE).}
% \vspace{-6mm}
% \label{tab:few_foundation}
% \end{table}

% \begin{table}[t]
% % \Huge
% \centering
% \renewcommand{\arraystretch}{0.6}%
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c||cc|cc}
% \toprule
% \textbf{N$\rightarrow$K}& 500 (N)             & 50 (N)              & 500 (N)             & 50 (N)              \\ \cmidrule{1-5}
% Ours+Midas    & 0.1885 / 0.0839 & 0.8017 / 0.0517 & 0.2059 / 0.0971 & 0.1910 / 0.8623 \\
% Ours+KBR      & 0.1769 / 0.0784 & 0.4153 / 0.2668 & 0.3103 / 0.2151 & 0.4971 / 0.3784 \\ \midrule
% \textbf{K$\rightarrow$N}& 64 (K)              & 8 (K)              & 64 (K)             & 8 (K)              \\ \cmidrule{1-5}
% Ours+Midas    & 1.2780 / 0.3486 & 4.8571 / 2.5653 & 1.9273 / 0.5875 & 6.3762 / 3.6092 \\
% Ours+KBR      & 1.2226 / 0.3324 & 4.2090 / 2.1382 & 1.8790 / 0.6192 & 5.1340 / 2.8451 \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-3.5mm}
% \caption{Few-shot cross-validation as in Tab.\textcolor{blue}{3}~(RMSE~/~MAE).}
% \vspace{-4mm}
% \label{tab:few_foundation}
% \end{table}

% \begin{table}[t]
% % \Huge
% \centering
% \renewcommand{\arraystretch}{0.8}%
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c||cc|cc}
% \toprule
%       % & \multicolumn{2}{c}{NYU -\textgreater KITTI} & \multicolumn{2}{c}{KITTI -\textgreater NYU}\\ \midrule
% \textbf{w/o Pretrain} & 64~(K)  & 8~(K)   & 500~(N) & 50  (N) \\ \midrule
% Ours+Midas  & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000         \\
% Ours+KBR    & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000        & 0.000~/~0.000         \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-3.5mm}
% \caption{Few-shot evaluation w/o pretraining in depth completion.}
% \vspace{-4mm}
% \label{tab:few_foundation}
% \end{table}

\begin{table}[t]
% \Huge
\centering
\renewcommand{\arraystretch}{0.8}%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c||cc|cc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c}{100-shot}      & \multicolumn{2}{c}{10-shot}       \\ \midrule
{(a)~Outdoor$\rightarrow$Indoor }& 500 (K$\rightarrow$N)             & 50 (K$\rightarrow$N)              & 500 (K$\rightarrow$N)             & 50 (K$\rightarrow$N)              \\ \cmidrule{1-5}
Ours+Midas~[\textcolor{blue}{5}]    & 0.189 / 0.084 & 0.594 / 0.411 & 0.206 / 0.097 & 0.810 / 0.661 \\
Ours+KBR~[\textcolor{blue}{59}]      & 0.177 / 0.078 & 0.415 / 0.267 & 0.310 / 0.215 & 0.497 / 0.378 \\ \midrule
{(b)~Indoor$\rightarrow$Outdoor}& 64 (N$\rightarrow$K)              & 8 (N$\rightarrow$K)              & 64 (N$\rightarrow$K)             & 8 (N$\rightarrow$K)              \\ \cmidrule{1-5}
Ours+Midas~[\textcolor{blue}{5}]    & 1.278 / 0.349 & 4.857 / 2.565 & 1.927 / 0.588 & 6.376 / 3.609 \\
Ours+KBR~[\textcolor{blue}{59}]      & 1.223 / 0.332 & 4.209 / 2.138 & 1.879 / 0.619 & 5.134 / 2.845 \\ \midrule
{(c)~w/o pretraining} & 64~(K)  & 500~(N)   & 8~(K) & 50  (N) \\ \midrule
Ours+Midas~[\textcolor{blue}{5}]  & 1.317 / 0.360        & 0.189 / 0.084        & 6.836 / 4.062        & 0.782 / 0.654         \\
Ours+KBR~[\textcolor{blue}{59}]    & 1.260 / 0.344        & 0.180 / 0.080        & 5.015 / 2.741        & 0.480 / 0.363         \\ \bottomrule
\end{tabular}%
}
\vspace{-3.8mm}
\caption{Few-shot evaluation of foundation models. (a),(b): cross-validation\,between\,in-/outdoor (c): w/o pretraining for N and K.}
\vspace{-6mm}
\label{tab:few_foundation}
\end{table}














==> tables/rebuttal_tab1.tex <==
\begin{table}[t]
% \LARGE
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c||ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
NYU   (\#Samles) & \multicolumn{3}{c}{200}                                                              & \multicolumn{3}{c}{100}                                                              & \multicolumn{3}{c}{32}                                                               & \multicolumn{3}{c}{8}                                                                & \multicolumn{3}{c}{4}                                                                & \multicolumn{3}{c}{1}                                                                \\ \cmidrule{1-19}
NLSPN            & \textbf{0.1428}            & \textbf{0.0633}            & \textbf{0.9885}            & 0.1783                     & 0.0892                     & 0.9811                     & 0.2709                     & 0.1541                     & 0.9479                     & 0.4335                     & 0.2898                     & 0.8581                     & 0.5102                     & 0.3636                     & 0.7905                     & 0.6489                     & 0.4911                     & 0.6816                     \\
C.Former & 0.1450                     & 0.0651                     & 0.9882                     & 0.1821                     & 0.0895                     & 0.9809                     & 0.2701                     & 0.1554                     & 0.9470                     & 0.4338                     & 0.2888                     & 0.8665                     & 0.5192                     & 0.3673                     & 0.7996                     & 0.6479                     & 0.4869                     & 0.7013                     \\
Ours             & 0.1435                     & 0.0642                     & 0.9881                     & \textbf{0.1778}            & \textbf{0.0870}            & \textbf{0.9812}            & \textbf{0.2472}            & \textbf{0.1452}            & \textbf{0.9546}            & \textbf{0.3673}            & \textbf{0.2464}            & \textbf{0.9133}            & \textbf{0.3827}            & \textbf{0.2627}            & \textbf{0.9031}            & \textbf{0.4040}            & \textbf{0.2848}            & \textbf{0.8935}            \\ \bottomrule
KITTI (\#Lines)  & \multicolumn{3}{c}{32}                                                               & \multicolumn{3}{c}{16}                                                               & \multicolumn{3}{c}{8}                                                                & \multicolumn{3}{c}{4}                                                                & \multicolumn{3}{c}{2}                                                                & \multicolumn{3}{c}{1}                                                                \\ \cmidrule{1-19}
NLSPN            & {1.2591} & {0.4403} & {0.9922} & {1.4878} & {0.5108} & {0.9901} & {1.8542} & {0.6601} & {0.9851} & {2.1721} & {0.8481} & {0.9766} & {2.4812} & {1.2186} & {0.9432} & {3.0790} & {1.4642} & {0.9240} \\
CompletionFormer & 1.9014                     & 0.6814                     & 0.9773                     & 2.1792                     & 0.7964                     & 0.9726                     & 2.6528                     & 0.9805                     & 0.9661                     & 3.2914                     & 1.3627                     & 0.9405                     & 3.7558                     & 1.7426                     & 0.9012                     & 5.4281                     & 2.4568                     & 0.8465                     \\
Ours             & \textbf{1.1465}            & \textbf{0.3472}            & \textbf{0.9942}            & \textbf{1.3512}            & \textbf{0.4134}            & \textbf{0.9922}            & \textbf{1.6419}            & \textbf{0.5470}            & \textbf{0.9888}            & \textbf{1.9507}            & \textbf{0.7629}            & \textbf{0.9809}            & \textbf{2.3841}            & \textbf{1.1976}            & \textbf{0.9505}            & \textbf{2.8234}            & \textbf{1.2678}            & \textbf{0.9535}            \\ \bottomrule
\end{tabular}%
}
\label{tab:ablation_RDA}
\end{table}



% \begin{table*}[!ht]
% \LARGE
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c||ccc|ccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{\# Lines} & \multicolumn{3}{c}{32}                                                               & \multicolumn{3}{c}{16}                                                               & \multicolumn{3}{c}{8}                                                                & \multicolumn{3}{c}{4}                                                                & \multicolumn{3}{c}{2}                                                                 & \multicolumn{3}{c}{1}                                                                 \\ \cmidrule{2-19}
%                           & RMSE                       & MAE                        &\!\!DELTA1\!\!                    & RMSE                       & MAE                        &\!\!DELTA1\!\!                    & RMSE                       & MAE                        &\!\!DELTA1\!\!                    & RMSE                       & MAE                        &\!\!DELTA1\!\!                    & RMSE                        & MAE                        &\!\!DELTA1\!\!                    & RMSE                        & MAE                        &\!\!DELTA1\!\!                    \\ \midrule
% CSPN                      & 1.3644                     & 0.4008                     & 0.9876                     & 2.0935                     & 0.7532                     & 0.9596                     & 3.5806                     & 1.6679                     & 0.8580                     & 5.7438                     & 3.1650                     & {0.6656} & 8.9143                      & 5.6544                     & 0.4478                     & 12.5666                     & 8.2679                     & 0.3379                     \\
% S2D                       & {1.8133} & {0.7426} & {0.9623} & {2.6886} & {1.1670} & {0.9232} & {4.5806} & {2.6697} & {0.6727} & {7.2951} & {4.9223} & {0.3866} & {10.1624} & {6.8438} & {0.2854} & {12.2972} & {7.9316} & {0.2057} \\
% NLSPN\dag                     & 1.1894                     & 0.3536                     & 0.9923                     & 1.9279                     & 0.6976                     & 0.9675                     & 3.2285                     & 1.5482                     & 0.8692                     & 4.7571                     & 2.5976                     & 0.7267                     & 6.0305                      & 3.8779                     & 0.4904                     & 8.8244                      & 5.2859                     & 0.3949                     \\
% DySPN                     & 1.6758 & 0.5449 & 0.9871 & 2.3979 & 0.9096 & 0.9624 & 3.4687 & 1.5774 & 0.883 & 5.2374 & 2.8549 & 0.6981 & 6.5413 & 4.0182 & 0.5118 & 9.5199 & 5.3260 & 0.4637  \\
% CompletionFormer\dag          & 1.2513                     & 0.3844                     & 0.9912                     & 2.1857                     & 0.8403                     & 0.9627                     & 3.6505                     & 1.7687                     & 0.8577                     & 6.2532                     & 3.4800                     & 0.6787                     & 8.9682                      & 5.9899                     & 0.4672                     & 12.7693                     & 9.0019                     & 0.3414                     \\ 
% SpAgNet                   & 1.6496                     & 0.7600                     & 0.9842                     & 2.2604                     & 1.0463                     & 0.9499                     & 3.8319                     & 2.0464                     & 0.7748                     & 6.8536                     & 3.8768                     & 0.5420                     & 8.7863                      & 5.9735                     & 0.3201                     & 11.5720                     & 6.4999                     & 0.4231                     \\ 
% SAN\dag  & 1.8188                     & 0.8160                     & 0.9793                     & 2.8866                     & 1.5915                     & 0.9087                     & 3.7936                     & 1.8339                     & 0.8967                     & 4.5894                     & 2.3092                     & 0.8523                     & 4.1416                      & 2.1280                     & 0.8591                     & 4.4444                      & 2.3270                     & 0.8153                     \\ \midrule
% Ours                      & \textbf{1.1465}            & \textbf{0.3472}            & \textbf{0.9942}            & \textbf{1.3512}            & \textbf{0.4134}            & \textbf{0.9922}            & \textbf{1.6419}            & \textbf{0.5470}            & \textbf{0.9888}            & \textbf{1.9507}            & \textbf{0.7629}            & \textbf{0.9809}            & \textbf{2.3841}             & \textbf{1.1976}            & \textbf{0.9505}            & \textbf{2.8234}             & \textbf{1.2678}            & \textbf{0.9535}            \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-4mm}
% \caption{Quantitative Results on KITTI DC. \dag~indicates that the publicly available code and weight are used in this experiment.}
% \vspace{-1mm}
% \end{table*}

==> tables/supple_tab_VOID_SUN.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\LARGE
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{c||ccc|ccc|ccc|ccc}
\toprule
                        & \multicolumn{3}{c}{VOID 150}                        & \multicolumn{3}{c}{VOID 500}                        & \multicolumn{3}{c}{VOID 1500}                       & \multicolumn{3}{c}{SUN-RGBD}                        \\ 
                        & RMSE            & MAE             & DELTA1          & RMSE            & MAE             & DELTA1          & RMSE            & MAE             & DELTA1          & RMSE            & MAE             & DELTA1          \\ \midrule
CSPN                    & 1.0747          & 0.7991          & 0.2745          & 0.7695          & 0.4776          & 0.4730           & 0.4046         & 0.2121         & 0.7286            & 0.5552          & 0.2464          & 0.8468          \\
NLSPN                   & 0.6964          & 0.5063          & 0.3572          & 0.4672          & 0.2853          & 0.5618          & 0.2563         & 0.1339         & 0.7801            & 0.5910          & 0.2665          & 0.8441          \\
CompletionFormer        & 0.8445          & 0.6976          & 0.2030          & 0.6090          & 0.4447          & 0.3541          & 0.3430         & 0.2158         & 0.5794            & 0.9615          & 0.8574          & 0.0564          \\
Ours                    & \textbf{0.1955} & \textbf{0.1358} & \textbf{0.7243} & \textbf{0.1637} & \textbf{0.1031} & \textbf{0.7457} & \textbf{0.1580} & \textbf{0.098} & \textbf{0.7582}   & \textbf{0.3962} & \textbf{0.2710} & \textbf{0.8402} \\ \bottomrule
\end{tabular}%
}
\vspace{-3mm}
\caption{Quantitative results on VOID and SUN-RGBD dataset.}
\label{tabl:void_sun}
\end{table*}

==> tables/tabl_ablation_tuning.tex <==
\begin{table}[]
\centering
\LARGE
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{c||ccc|ccc}
\toprule
            & \multicolumn{3}{c}{Sparsity (500\!\rightarrow\!50)} & \multicolumn{3}{c}{Sparsity Rev.   (50\!\rightarrow\!500)}                                                       \\ \cmidrule{2-7}
            & RMSE            & MAE             & DELTA1          & {RMSE}            & {MAE}             & {DELTA1}          \\ \midrule
PT          & 0.4932 & 0.3231 & 0.7305 & 0.1542 & 0.6797 & 0.9856          \\
PT + BT     & 0.4367 & 0.272  & 0.8602 & 0.1503 & 0.6657 & 0.9862          \\
PTE         & 0.4735 & 0.3001 & 0.8553 & 0.1596 & 0.6966 & 0.9852          \\
PTE + BT    & 0.4105 & 0.2536 & 0.8771 & 0.1551 & 0.687  & 0.9851          \\
AD          & 0.4773 & 0.3062 & 0.8445 & 0.1769 & 0.8169 & 0.9808          \\
AD + BT     & 0.4699 & 0.2964 & 0.8496 & 0.1642 & 0.7425 & 0.9827          \\ \midrule
\textbf{BT} & \textbf{0.3997} & \textbf{0.2418} & \textbf{0.8825} & {\textbf{0.1453}} & {\textbf{0.6340}} & {\textbf{0.9874}} \\ \bottomrule
\end{tabular}%
}
\vspace{-3.5mm}
\caption{Ablation on tuning protocols. We compare soft prompt tuning~(PT)~\cite{jia2022visual}, prompt tuning express~(PTE)~\cite{razdaibiedina2023residual}, adapter~\cite{chen2022adaptformer}, and bias tuning (BT)~\cite{cai2020tinytl}.}
\vspace{-3.5mm}
\label{tab:tuning}
\end{table}
